Factored Task and Motion Planning with Combined Optimization, Sampling and Learning

In this thesis, we aim to improve the performance of TAMP algorithms from three complementary perspectives. First, we investigate the integration of discrete task planning with continuous trajectory optimization. Our main contribution is a conflict-based solver that automatically discovers why a task plan might fail when considering the constraints of the physical world. This information is then fed back into the task planner, resulting in an efficient, bidirectional, and intuitive interface between task and motion, capable of solving TAMP problems with multiple objects, robots, and tight physical constraints. In the second part, we first illustrate that, given the wide range of tasks and environments within TAMP, neither sampling nor optimization is superior in all settings. To combine the strengths of both approaches, we have designed meta-solvers for TAMP, adaptive solvers that automatically select which algorithms and computations to use and how to best decompose each problem to find a solution faster. In the third part, we combine deep learning architectures with model-based reasoning to accelerate computations within our TAMP solver. Specifically, we target infeasibility detection and nonlinear optimization, focusing on generalization, accuracy, compute time, and data efficiency. At the core of our contributions is a refined, factored representation of the trajectory optimization problems inside TAMP. This structure not only facilitates more efficient planning, encoding of geometric infeasibility, and meta-reasoning but also provides better generalization in neural architectures.

==> afafdfa <==
\begin{tabular}{||l|l||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||c|c|c||}
\hline
\# & Problem & \multicolumn{3}{c||}{Opt} & \multicolumn{3}{c||}{Sampling} & \multicolumn{3}{c||}{Meta}\\
\hline
 &  & $Q_1$ & $Q_2$ & $Q_3$ & $Q_1$ & $Q_2$ & $Q_3$ & $Q_1$ & $Q_2$ & $Q_3$\\
\hline
1 & handover & \textcolor{ForestGreen}{0.9} & 1.2 & 1.4 & \textcolor{Red}{1.0} & \textcolor{Red}{2.7} & \textcolor{Red}{7.0} & 0.9 & \textcolor{ForestGreen}{1.0} & \textcolor{ForestGreen}{1.1}\\
\hline
2 & small & \textcolor{ForestGreen}{0.7} & \textcolor{ForestGreen}{1.0} & \textcolor{ForestGreen}{2.3} & \textcolor{Red}{2.9} & \textcolor{Red}{5.8} & \textcolor{Red}{11.3} & 1.6 & 2.4 & 3.3\\
\hline
3 & cluttered & \textcolor{Red}{2.1} & \textcolor{Red}{3.4} & \textcolor{Red}{8.8} & \textcolor{ForestGreen}{0.6} & \textcolor{ForestGreen}{1.0} & \textcolor{ForestGreen}{1.5} & 0.7 & 2.1 & 2.9\\
\hline
4 & stack & \textcolor{Red}{1.3} & \textcolor{Red}{1.9} & \textcolor{Red}{2.6} & 0.9 & 1.0 & \textcolor{ForestGreen}{1.1} & \textcolor{ForestGreen}{0.9} & \textcolor{ForestGreen}{1.0} & 1.2\\
\hline
5 & occupied & \textcolor{ForestGreen}{0.7} & \textcolor{ForestGreen}{1.0} & \textcolor{ForestGreen}{1.5} & 1.6 & \textcolor{Red}{4.6} & \textcolor{Red}{5.9} & \textcolor{Red}{1.7} & 1.9 & 2.2\\
\hline
6 & transfer & 1.2 & 1.8 & 2.1 & \textcolor{Red}{1.5} & \textcolor{Red}{2.8} & \textcolor{Red}{4.4} & \textcolor{ForestGreen}{0.8} & \textcolor{ForestGreen}{1.0} & \textcolor{ForestGreen}{1.3}\\
\hline
7 & transfer-obs & \textcolor{Red}{5.1} & \textcolor{Red}{5.7} & \textcolor{Red}{9.1} & \textcolor{ForestGreen}{0.9} & \textcolor{ForestGreen}{1.0} & \textcolor{ForestGreen}{1.1} & 2.0 & 2.6 & 2.9\\
\hline
\hline
 & Summary & 1.7 & 2.3 & 4.0 & 1.3 & 2.7 & 4.6 & 1.2 & 1.7 & 2.1\\
\hline
\end{tabular}


==> bench/pp-bench/r0.tex <==
\makeatletter\newcommand\rawzero[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@out{\{"error": {[}1.21, 1.35{]}, "f\_dist1": {[}0.53, 0.14{]}, "f\_dist2": {[}0.79, 0.12{]}, "p\_dist1": {[}0.22, 0.12{]}, "p\_dist2": {[}0.29, 0.1{]}, "q\_dist1": {[}0.29, 0.07{]}, "q\_dist2": {[}0.5, 0.07{]}, "t\_dist1": {[}0.23, 0.11{]}, "t\_dist2": {[}0.26, 0.11{]}\}}\else\ifnum\pdfstrcmp{#1}{error}=0\let\rawzero@out\rawzero@I\else\ifnum\pdfstrcmp{#1}{f_dist1}=0\let\rawzero@out\rawzero@II\else\ifnum\pdfstrcmp{#1}{f_dist2}=0\let\rawzero@out\rawzero@III\else\ifnum\pdfstrcmp{#1}{p_dist1}=0\let\rawzero@out\rawzero@IV\else\ifnum\pdfstrcmp{#1}{p_dist2}=0\let\rawzero@out\rawzero@V\else\ifnum\pdfstrcmp{#1}{q_dist1}=0\let\rawzero@out\rawzero@VI\else\ifnum\pdfstrcmp{#1}{q_dist2}=0\let\rawzero@out\rawzero@VII\else\ifnum\pdfstrcmp{#1}{t_dist1}=0\let\rawzero@out\rawzero@VIII\else\ifnum\pdfstrcmp{#1}{t_dist2}=0\let\rawzero@out\rawzero@IX\else\def\rawzero@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\rawzero@out}\newcommand\rawzero@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@I@out{{[}1.21, 1.35{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawzero@I@out{1.21}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawzero@I@out{1.35}\else\def\rawzero@I@out{??}\fi\fi\fi\rawzero@I@out}\newcommand\rawzero@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@II@out{{[}0.53, 0.14{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawzero@II@out{0.53}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawzero@II@out{0.14}\else\def\rawzero@II@out{??}\fi\fi\fi\rawzero@II@out}\newcommand\rawzero@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@III@out{{[}0.79, 0.12{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawzero@III@out{0.79}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawzero@III@out{0.12}\else\def\rawzero@III@out{??}\fi\fi\fi\rawzero@III@out}\newcommand\rawzero@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@IV@out{{[}0.22, 0.12{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawzero@IV@out{0.22}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawzero@IV@out{0.12}\else\def\rawzero@IV@out{??}\fi\fi\fi\rawzero@IV@out}\newcommand\rawzero@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@V@out{{[}0.29, 0.1{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawzero@V@out{0.29}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawzero@V@out{0.1}\else\def\rawzero@V@out{??}\fi\fi\fi\rawzero@V@out}\newcommand\rawzero@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@VI@out{{[}0.29, 0.07{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawzero@VI@out{0.29}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawzero@VI@out{0.07}\else\def\rawzero@VI@out{??}\fi\fi\fi\rawzero@VI@out}\newcommand\rawzero@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@VII@out{{[}0.5, 0.07{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawzero@VII@out{0.5}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawzero@VII@out{0.07}\else\def\rawzero@VII@out{??}\fi\fi\fi\rawzero@VII@out}\newcommand\rawzero@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@VIII@out{{[}0.23, 0.11{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawzero@VIII@out{0.23}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawzero@VIII@out{0.11}\else\def\rawzero@VIII@out{??}\fi\fi\fi\rawzero@VIII@out}\newcommand\rawzero@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawzero@IX@out{{[}0.26, 0.11{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawzero@IX@out{0.26}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawzero@IX@out{0.11}\else\def\rawzero@IX@out{??}\fi\fi\fi\rawzero@IX@out}\makeatother


==> bench/pp-bench/r1.tex <==
\makeatletter\newcommand\rawone[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@out{\{"error": {[}1.46, 0.79{]}, "f\_dist1": {[}0.47, 0.13{]}, "f\_dist2": {[}0.57, 0.08{]}, "p\_dist1": {[}0.25, 0.12{]}, "p\_dist2": {[}0.14, 0.04{]}, "q\_dist1": {[}0.21, 0.07{]}, "q\_dist2": {[}0.37, 0.05{]}, "t\_dist1": {[}0.17, 0.07{]}, "t\_dist2": {[}0.14, 0.04{]}\}}\else\ifnum\pdfstrcmp{#1}{error}=0\let\rawone@out\rawone@I\else\ifnum\pdfstrcmp{#1}{f_dist1}=0\let\rawone@out\rawone@II\else\ifnum\pdfstrcmp{#1}{f_dist2}=0\let\rawone@out\rawone@III\else\ifnum\pdfstrcmp{#1}{p_dist1}=0\let\rawone@out\rawone@IV\else\ifnum\pdfstrcmp{#1}{p_dist2}=0\let\rawone@out\rawone@V\else\ifnum\pdfstrcmp{#1}{q_dist1}=0\let\rawone@out\rawone@VI\else\ifnum\pdfstrcmp{#1}{q_dist2}=0\let\rawone@out\rawone@VII\else\ifnum\pdfstrcmp{#1}{t_dist1}=0\let\rawone@out\rawone@VIII\else\ifnum\pdfstrcmp{#1}{t_dist2}=0\let\rawone@out\rawone@IX\else\def\rawone@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\rawone@out}\newcommand\rawone@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@I@out{{[}1.46, 0.79{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawone@I@out{1.46}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawone@I@out{0.79}\else\def\rawone@I@out{??}\fi\fi\fi\rawone@I@out}\newcommand\rawone@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@II@out{{[}0.47, 0.13{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawone@II@out{0.47}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawone@II@out{0.13}\else\def\rawone@II@out{??}\fi\fi\fi\rawone@II@out}\newcommand\rawone@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@III@out{{[}0.57, 0.08{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawone@III@out{0.57}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawone@III@out{0.08}\else\def\rawone@III@out{??}\fi\fi\fi\rawone@III@out}\newcommand\rawone@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@IV@out{{[}0.25, 0.12{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawone@IV@out{0.25}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawone@IV@out{0.12}\else\def\rawone@IV@out{??}\fi\fi\fi\rawone@IV@out}\newcommand\rawone@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@V@out{{[}0.14, 0.04{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawone@V@out{0.14}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawone@V@out{0.04}\else\def\rawone@V@out{??}\fi\fi\fi\rawone@V@out}\newcommand\rawone@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@VI@out{{[}0.21, 0.07{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawone@VI@out{0.21}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawone@VI@out{0.07}\else\def\rawone@VI@out{??}\fi\fi\fi\rawone@VI@out}\newcommand\rawone@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@VII@out{{[}0.37, 0.05{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawone@VII@out{0.37}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawone@VII@out{0.05}\else\def\rawone@VII@out{??}\fi\fi\fi\rawone@VII@out}\newcommand\rawone@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@VIII@out{{[}0.17, 0.07{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawone@VIII@out{0.17}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawone@VIII@out{0.07}\else\def\rawone@VIII@out{??}\fi\fi\fi\rawone@VIII@out}\newcommand\rawone@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawone@IX@out{{[}0.14, 0.04{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawone@IX@out{0.14}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawone@IX@out{0.04}\else\def\rawone@IX@out{??}\fi\fi\fi\rawone@IX@out}\makeatother


==> bench/pp-bench/r2.tex <==
\makeatletter\newcommand\rawtwo[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@out{\{"error": {[}8.38, 1.82{]}, "f\_dist1": {[}0.7, 0.11{]}, "f\_dist2": {[}0.81, 0.09{]}, "p\_dist1": {[}0.24, 0.08{]}, "p\_dist2": {[}0.25, 0.07{]}, "q\_dist1": {[}0.4, 0.07{]}, "q\_dist2": {[}0.49, 0.05{]}, "t\_dist1": {[}0.33, 0.07{]}, "t\_dist2": {[}0.32, 0.08{]}\}}\else\ifnum\pdfstrcmp{#1}{error}=0\let\rawtwo@out\rawtwo@I\else\ifnum\pdfstrcmp{#1}{f_dist1}=0\let\rawtwo@out\rawtwo@II\else\ifnum\pdfstrcmp{#1}{f_dist2}=0\let\rawtwo@out\rawtwo@III\else\ifnum\pdfstrcmp{#1}{p_dist1}=0\let\rawtwo@out\rawtwo@IV\else\ifnum\pdfstrcmp{#1}{p_dist2}=0\let\rawtwo@out\rawtwo@V\else\ifnum\pdfstrcmp{#1}{q_dist1}=0\let\rawtwo@out\rawtwo@VI\else\ifnum\pdfstrcmp{#1}{q_dist2}=0\let\rawtwo@out\rawtwo@VII\else\ifnum\pdfstrcmp{#1}{t_dist1}=0\let\rawtwo@out\rawtwo@VIII\else\ifnum\pdfstrcmp{#1}{t_dist2}=0\let\rawtwo@out\rawtwo@IX\else\def\rawtwo@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\rawtwo@out}\newcommand\rawtwo@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@I@out{{[}8.38, 1.82{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawtwo@I@out{8.38}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawtwo@I@out{1.82}\else\def\rawtwo@I@out{??}\fi\fi\fi\rawtwo@I@out}\newcommand\rawtwo@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@II@out{{[}0.7, 0.11{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawtwo@II@out{0.7}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawtwo@II@out{0.11}\else\def\rawtwo@II@out{??}\fi\fi\fi\rawtwo@II@out}\newcommand\rawtwo@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@III@out{{[}0.81, 0.09{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawtwo@III@out{0.81}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawtwo@III@out{0.09}\else\def\rawtwo@III@out{??}\fi\fi\fi\rawtwo@III@out}\newcommand\rawtwo@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@IV@out{{[}0.24, 0.08{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawtwo@IV@out{0.24}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawtwo@IV@out{0.08}\else\def\rawtwo@IV@out{??}\fi\fi\fi\rawtwo@IV@out}\newcommand\rawtwo@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@V@out{{[}0.25, 0.07{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawtwo@V@out{0.25}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawtwo@V@out{0.07}\else\def\rawtwo@V@out{??}\fi\fi\fi\rawtwo@V@out}\newcommand\rawtwo@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@VI@out{{[}0.4, 0.07{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawtwo@VI@out{0.4}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawtwo@VI@out{0.07}\else\def\rawtwo@VI@out{??}\fi\fi\fi\rawtwo@VI@out}\newcommand\rawtwo@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@VII@out{{[}0.49, 0.05{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawtwo@VII@out{0.49}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawtwo@VII@out{0.05}\else\def\rawtwo@VII@out{??}\fi\fi\fi\rawtwo@VII@out}\newcommand\rawtwo@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@VIII@out{{[}0.33, 0.07{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawtwo@VIII@out{0.33}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawtwo@VIII@out{0.07}\else\def\rawtwo@VIII@out{??}\fi\fi\fi\rawtwo@VIII@out}\newcommand\rawtwo@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawtwo@IX@out{{[}0.32, 0.08{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawtwo@IX@out{0.32}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawtwo@IX@out{0.08}\else\def\rawtwo@IX@out{??}\fi\fi\fi\rawtwo@IX@out}\makeatother


==> bench/pp-bench/r3.tex <==
\makeatletter\newcommand\rawthree[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@out{\{"error": {[}8.09, 1.35{]}, "f\_dist1": {[}0.62, 0.1{]}, "f\_dist2": {[}0.6, 0.08{]}, "p\_dist1": {[}0.26, 0.13{]}, "p\_dist2": {[}0.16, 0.07{]}, "q\_dist1": {[}0.38, 0.04{]}, "q\_dist2": {[}0.38, 0.04{]}, "t\_dist1": {[}0.19, 0.05{]}, "t\_dist2": {[}0.16, 0.04{]}\}}\else\ifnum\pdfstrcmp{#1}{error}=0\let\rawthree@out\rawthree@I\else\ifnum\pdfstrcmp{#1}{f_dist1}=0\let\rawthree@out\rawthree@II\else\ifnum\pdfstrcmp{#1}{f_dist2}=0\let\rawthree@out\rawthree@III\else\ifnum\pdfstrcmp{#1}{p_dist1}=0\let\rawthree@out\rawthree@IV\else\ifnum\pdfstrcmp{#1}{p_dist2}=0\let\rawthree@out\rawthree@V\else\ifnum\pdfstrcmp{#1}{q_dist1}=0\let\rawthree@out\rawthree@VI\else\ifnum\pdfstrcmp{#1}{q_dist2}=0\let\rawthree@out\rawthree@VII\else\ifnum\pdfstrcmp{#1}{t_dist1}=0\let\rawthree@out\rawthree@VIII\else\ifnum\pdfstrcmp{#1}{t_dist2}=0\let\rawthree@out\rawthree@IX\else\def\rawthree@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\rawthree@out}\newcommand\rawthree@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@I@out{{[}8.09, 1.35{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawthree@I@out{8.09}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawthree@I@out{1.35}\else\def\rawthree@I@out{??}\fi\fi\fi\rawthree@I@out}\newcommand\rawthree@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@II@out{{[}0.62, 0.1{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawthree@II@out{0.62}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawthree@II@out{0.1}\else\def\rawthree@II@out{??}\fi\fi\fi\rawthree@II@out}\newcommand\rawthree@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@III@out{{[}0.6, 0.08{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawthree@III@out{0.6}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawthree@III@out{0.08}\else\def\rawthree@III@out{??}\fi\fi\fi\rawthree@III@out}\newcommand\rawthree@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@IV@out{{[}0.26, 0.13{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawthree@IV@out{0.26}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawthree@IV@out{0.13}\else\def\rawthree@IV@out{??}\fi\fi\fi\rawthree@IV@out}\newcommand\rawthree@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@V@out{{[}0.16, 0.07{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawthree@V@out{0.16}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawthree@V@out{0.07}\else\def\rawthree@V@out{??}\fi\fi\fi\rawthree@V@out}\newcommand\rawthree@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@VI@out{{[}0.38, 0.04{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawthree@VI@out{0.38}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawthree@VI@out{0.04}\else\def\rawthree@VI@out{??}\fi\fi\fi\rawthree@VI@out}\newcommand\rawthree@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@VII@out{{[}0.38, 0.04{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawthree@VII@out{0.38}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawthree@VII@out{0.04}\else\def\rawthree@VII@out{??}\fi\fi\fi\rawthree@VII@out}\newcommand\rawthree@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@VIII@out{{[}0.19, 0.05{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawthree@VIII@out{0.19}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawthree@VIII@out{0.05}\else\def\rawthree@VIII@out{??}\fi\fi\fi\rawthree@VIII@out}\newcommand\rawthree@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\rawthree@IX@out{{[}0.16, 0.04{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\rawthree@IX@out{0.16}\else\ifnum\pdfstrcmp{#1}{1}=0\def\rawthree@IX@out{0.04}\else\def\rawthree@IX@out{??}\fi\fi\fi\rawthree@IX@out}\makeatother


==> bench/pp-bench/s0.tex <==
\makeatletter\newcommand\solzero[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\solzero@out{\{"f\_dist1": {[}0.41, 0.13{]}, "f\_dist2": {[}0.75, 0.13{]}\}}\else\ifnum\pdfstrcmp{#1}{f_dist1}=0\let\solzero@out\solzero@I\else\ifnum\pdfstrcmp{#1}{f_dist2}=0\let\solzero@out\solzero@II\else\def\solzero@out{??}\fi\fi\fi\solzero@out}\newcommand\solzero@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\solzero@I@out{{[}0.41, 0.13{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\solzero@I@out{0.41}\else\ifnum\pdfstrcmp{#1}{1}=0\def\solzero@I@out{0.13}\else\def\solzero@I@out{??}\fi\fi\fi\solzero@I@out}\newcommand\solzero@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\solzero@II@out{{[}0.75, 0.13{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\solzero@II@out{0.75}\else\ifnum\pdfstrcmp{#1}{1}=0\def\solzero@II@out{0.13}\else\def\solzero@II@out{??}\fi\fi\fi\solzero@II@out}\makeatother


==> bench/pp-bench/s1.tex <==
\makeatletter\newcommand\solone[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\solone@out{\{"f\_dist1": {[}0.28, 0.08{]}, "f\_dist2": {[}0.44, 0.07{]}\}}\else\ifnum\pdfstrcmp{#1}{f_dist1}=0\let\solone@out\solone@I\else\ifnum\pdfstrcmp{#1}{f_dist2}=0\let\solone@out\solone@II\else\def\solone@out{??}\fi\fi\fi\solone@out}\newcommand\solone@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\solone@I@out{{[}0.28, 0.08{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\solone@I@out{0.28}\else\ifnum\pdfstrcmp{#1}{1}=0\def\solone@I@out{0.08}\else\def\solone@I@out{??}\fi\fi\fi\solone@I@out}\newcommand\solone@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\solone@II@out{{[}0.44, 0.07{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\solone@II@out{0.44}\else\ifnum\pdfstrcmp{#1}{1}=0\def\solone@II@out{0.07}\else\def\solone@II@out{??}\fi\fi\fi\solone@II@out}\makeatother


==> bench/pp-bench/s2.tex <==
\makeatletter\newcommand\soltwo[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\soltwo@out{\{"f\_dist1": {[}0.39, 0.06{]}, "f\_dist2": {[}0.58, 0.12{]}\}}\else\ifnum\pdfstrcmp{#1}{f_dist1}=0\let\soltwo@out\soltwo@I\else\ifnum\pdfstrcmp{#1}{f_dist2}=0\let\soltwo@out\soltwo@II\else\def\soltwo@out{??}\fi\fi\fi\soltwo@out}\newcommand\soltwo@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\soltwo@I@out{{[}0.39, 0.06{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\soltwo@I@out{0.39}\else\ifnum\pdfstrcmp{#1}{1}=0\def\soltwo@I@out{0.06}\else\def\soltwo@I@out{??}\fi\fi\fi\soltwo@I@out}\newcommand\soltwo@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\soltwo@II@out{{[}0.58, 0.12{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\soltwo@II@out{0.58}\else\ifnum\pdfstrcmp{#1}{1}=0\def\soltwo@II@out{0.12}\else\def\soltwo@II@out{??}\fi\fi\fi\soltwo@II@out}\makeatother


==> bench/pp-bench/s3.tex <==
\makeatletter\newcommand\solthree[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\solthree@out{\{"f\_dist1": {[}0.44, 0.06{]}, "f\_dist2": {[}0.41, 0.05{]}\}}\else\ifnum\pdfstrcmp{#1}{f_dist1}=0\let\solthree@out\solthree@I\else\ifnum\pdfstrcmp{#1}{f_dist2}=0\let\solthree@out\solthree@II\else\def\solthree@out{??}\fi\fi\fi\solthree@out}\newcommand\solthree@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\solthree@I@out{{[}0.44, 0.06{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\solthree@I@out{0.44}\else\ifnum\pdfstrcmp{#1}{1}=0\def\solthree@I@out{0.06}\else\def\solthree@I@out{??}\fi\fi\fi\solthree@I@out}\newcommand\solthree@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\solthree@II@out{{[}0.41, 0.05{]}}\else\ifnum\pdfstrcmp{#1}{0}=0\def\solthree@II@out{0.41}\else\ifnum\pdfstrcmp{#1}{1}=0\def\solthree@II@out{0.05}\else\def\solthree@II@out{??}\fi\fi\fi\solthree@II@out}\makeatother

